SuMe: A Dataset Towards Summarizing Biomedical Mechanisms

Can language models read biomedical texts and explain the biomedical mechanisms discussed? In this work we introduce a biomedical mechanism summarization task. Biomedical studies often investigate the mechanisms behind how one entity (e.g., a protein or a chemical) affects another in a biological context. The abstracts of these publications often include a focused set of sentences that present relevant supporting statements regarding such relationships, associated experimental evidence, and a concluding sentence that summarizes the mechanism underlying the relationship. We leverage this structure and create a summarization task, where the input is a collection of sentences and the main entities in an abstract, and the output includes the relationship and a sentence that summarizes the mechanism. Using a small amount of manually labeled mechanism sentences, we train a mechanism sentence classifier to filter a large biomedical abstract collection and create a summarization dataset with 22k instances. We also introduce conclusion sentence generation as a pretraining task with 611k instances. We benchmark the performance of large bio-domain language models. We find that while the pretraining task help improves performance, the best model produces acceptable mechanism outputs in only 32% of the instances, which shows the task presents significant challenges in biomedical language understanding and summarization.

==> modeling.tex <==
\section{Modeling}
\label{modeling}

\subsection{Data Augmentation}
We pretrained the transformer based models with a set of 611k abstracts from pubmed database. We follow the same framework in section~\ref{task} to create this dataset but we include all the abstracts both the ones ending with mechanism sentences and the one ending with non mechanism sentences. We also skip entity-relation extraction to focus on summarization task more than relation extraction. 


\subsection{Supporting Sentence Selection}
Abstracts usually consist of many sentences which might not play the same role on the final conclusion. On the other hand, many transformer based models are restricted in the number of tokens as inputs. We analyze whether selecting most important sentences can be helpful to generate the explanation or not. For this purpose, we compute the similarity between the conclusion sentence and each sentence in the supporting set, retrain the model with the most similar sentence to the mechanism sentence and evaluate the effectiveness of similarity of supporting sentences and the conclusion sentence. 


\subsection{Reranking the Generation using Mechanisms}
We also evaluate the effectiveness of rescoring the mechanism sentence generation by using mechanism sentence classifier. Given the trained models, for each sentence we generate a number of possible outputs as diverse as possible using beam search and then select the best generation based on their mechanism sentence score.

